ZEN 2.0: Continue Training and Adaption for N-gram Enhanced Text Encoders

Pre-trained text encoders have drawn sustaining attention in natural language processing (NLP) and shown their capability in obtaining promising results in different tasks. Recent studies illustrated that external self-supervised signals (or knowledge extracted by unsupervised learning, such as n-grams) are beneficial to provide useful semantic evidence for understanding languages such as Chinese, so as to improve the performance on various downstream tasks accordingly. To further enhance the encoders, in this paper, we propose to pre-train n-gram-enhanced encoders with a large volume of data and advanced techniques for training. Moreover, we try to extend the encoder to different languages as well as different domains, where it is confirmed that the same architecture is applicable to these varying circumstances and new state-of-the-art performance is observed from a long list of NLP tasks across languages and domains.

==> tables/analysis_adapted.tex <==

\begin{table*}[h]
\begin{center}
\begin{small}
\begin{tabular}{p{1.84cm}
                   C{1.5cm} 
                   C{1.6cm} 
                   C{1.98cm}  
                   C{1.7cm} 
                   C{1.8cm} 
                   C{2.4cm} }
\toprule
\multirow{3}*{\textbf{}}
&\multirow{3}*{\textbf{Adapted}}
&\multicolumn{1}{c}{\textsc{\textbf {CWS}}}
&\multicolumn{1}{c}{\textsc{\textbf{POS tagging}}}
&\multicolumn{1}{c}{\textsc{\textbf{NER}}}
&\multicolumn{1}{c}{\textsc{\textbf{DC}}}
&\multicolumn{1}{c}{\textsc{\textbf{SA}}}\\
\addlinespace[0.05cm]
\cline{3-7}
\addlinespace[0.05cm]
~& ~
&\multicolumn{1}{c}{\textsc{\textbf {MSR-CWS}}}
&\multicolumn{1}{c}{\textsc{\textbf{CTB5}}}
&\multicolumn{1}{c}{\textsc{\textbf{MSRA-NER}}}
&\multicolumn{1}{c}{\textsc{\textbf{THUCNews}}}
&\multicolumn{1}{c}{\textsc{\textbf{ChnSentiCorp}}}\\
\addlinespace[0.05cm]
\cline{3-7}
\addlinespace[0.05cm]
~& ~&
\multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} \\
\midrule	
% Vanilla ZEN (B) & 98.29 & 96.84 & 94.74 & 97.63 & \textbf{96.08} \\
% Adapted ZEN (B) & \textbf{98.41} & \textbf{97.00} & \textbf{95.54} & \textbf{97.64} & \textbf{96.08} \\
% \midrule
\multirow{2}*{ZEN 2.0 (L)} & \multicolumn{1}{c}{$\surd$} & \textbf{98.66} & \textbf{97.09} & \textbf{96.20} & \textbf{97.93} & \textbf{96.50} \\
& \multicolumn{1}{c}{$\texttimes$} & 98.51 & 97.05 & 96.25 & 97.81 & 96.42 \\
\bottomrule
\end{tabular}
\begin{tabular}{p{1.9cm}
                   C{1.5cm} 
                   C{1.8cm} 
                   C{1.8cm} 
                   C{1.8cm} 
                   C{2.0cm} 
                   C{2.2cm} }
\toprule
\multirow{3}*{\textbf{}}
&\multirow{3}*{\textbf{Adapted}}
&\multicolumn{2}{c}{\textsc{\textbf{SPM}}}
&\multicolumn{1}{c}{\textsc{\textbf{NLI}}}
&\multicolumn{1}{c}{\textsc{\textbf{MRC}}}
&\multicolumn{1}{c}{\textsc{\textbf{QA}}}\\
\addlinespace[0.05cm]
\cline{3-7}
\addlinespace[0.05cm]
~& ~
&\multicolumn{1}{c}{\textsc{\textbf{LCQMC}}}
&\multicolumn{1}{c}{\textsc{\textbf{BQ Corpus}}}
&\multicolumn{1}{c}{\textsc{\textbf{XNLI}}}
&\multicolumn{1}{c}{\textsc{\textbf{CMRC2018}}}
&\multicolumn{1}{c}{\textsc{\textbf{NLPCC-DBQA}}}\\
\addlinespace[0.05cm]
\cline{3-7}
\addlinespace[0.05cm]
~& ~&
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{EM/F1}} &
\multicolumn{1}{c}{\small{MRR/F1}} \\
\midrule	
% Vanilla ZEN (B) & 87.66 & 85.66 & 78.98 & 69.21/86.91 & 95.13/82.85 \\
% Adapted ZEN (B) & \textbf{88.39} & \textbf{85.65} & \textbf{80.28} & \textbf{70.77/87.97} & \textbf{95.74/84.43} \\
% \midrule
\multirow{2}*{ZEN 2.0 (L)} & \multicolumn{1}{c}{$\surd$} & \textbf{88.81} & \textbf{85.99} & \textbf{83.09} & \textbf{73.00/89.92} & \textbf{96.11/86.47} \\
& \multicolumn{1}{c}{$\texttimes$}& 88.44 & 85.70 & 82.59 & 72.32/89.51 & 96.04/86.08 \\
\bottomrule
\end{tabular}
\end{small}
\vspace{-0.3cm}
\end{center}
\caption{\label{result-adapted-zh-table} 
\textcolor{blue}{The results of fine-tuning Chinese ZEN 2.0 with and without adapted character encoder on different tasks.} 
% Only CMRC2018 dataset reports the result of development dataset, the other datasets report the results of test dataset.
}
\vskip -1em
\end{table*}


==> tables/analysis_ngram.tex <==



\begin{table*}[h]
\begin{center}
\begin{small}
\begin{tabular}{p{1.8cm}
                   C{1.2cm} 
                   C{1.8cm} 
                   C{1.78cm}  
                   C{1.9cm} 
                   C{1.9cm} 
                   C{2.6cm} }
\toprule
\multirow{2}*{\textbf{}}
&\multirow{2}*{\textbf{N-gram}}
&\multicolumn{1}{c}{\textsc{\textbf {MSR-CWS}}}
&\multicolumn{1}{c}{\textsc{\textbf{CTB5}}}
&\multicolumn{1}{c}{\textsc{\textbf{MSRA-NER}}}
&\multicolumn{1}{c}{\textsc{\textbf{THUCNews}}}
&\multicolumn{1}{c}{\textsc{\textbf{ChnSentiCorp}}}\\
\addlinespace[0.05cm]
\cline{3-7}
\addlinespace[0.05cm]
~& ~& 
\multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} \\
\midrule
\multirow{2}*{ZEN 2.0 (B)} & \multicolumn{1}{c}{$\surd$} & \textbf{98.41} & \textbf{97.00} & \textbf{95.54} & \textbf{97.64} & \textbf{96.08} \\
 & \multicolumn{1}{c}{$\texttimes$} & 98.29 & 96.53 & 95.08 & 97.56 & 96.00 \\
\midrule
\multirow{2}*{ZEN 2.0 (L)} & \multicolumn{1}{c}{$\surd$} & \textbf{98.66} & \textbf{97.09} & \textbf{96.20} & \textbf{97.93} & \textbf{96.50} \\
 & \multicolumn{1}{c}{$\texttimes$} & 98.54 & 96.71 & 95.79 & 97.72 & 96.18 \\
\bottomrule
\end{tabular}

\begin{tabular}{p{1.8cm}
                   C{1.2cm} 
                   C{1.8cm} 
                   C{1.9cm} 
                   C{1.8cm} 
                   C{1.98cm} 
                   C{2.5cm} }
\toprule
\multirow{2}*{\textbf{}}
&\multirow{2}*{\textbf{N-gram}}
&\multicolumn{1}{c}{\textsc{\textbf{LCQMC}}}
&\multicolumn{1}{c}{\textsc{\textbf{BQ Corpus}}}
&\multicolumn{1}{c}{\textsc{\textbf{NLI}}}
&\multicolumn{1}{c}{\textsc{\textbf{CMRC2018}}}
&\multicolumn{1}{c}{\textsc{\textbf{NLPCC-DBQA}}}\\
\addlinespace[0.05cm]
\cline{3-7}
\addlinespace[0.05cm]
~& ~& 
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{EM/F1}} &
\multicolumn{1}{c}{\small{MRR/F1}} \\
\midrule	
\multirow{2}*{ZEN 2.0 (B)} & \multicolumn{1}{c}{$\surd$} & \textbf{88.71} & \textbf{85.65} & \textbf{79.30} & \textbf{70.77/87.97} & \textbf{95.74/84.43} \\
 & \multicolumn{1}{c}{$\texttimes$} & 87.82 & 85.23 & 78.78 & 69.56/86.72 & 95.17/84.34 \\
\midrule
\multirow{2}*{ZEN 2.0 (L)} & \multicolumn{1}{c}{$\surd$} & \textbf{88.81} & \textbf{85.99} & \textbf{83.09} & \textbf{73.00/89.92} & \textbf{96.11/86.47} \\
 & \multicolumn{1}{c}{$\texttimes$} & 88.53 & 85.87 & 82.30 & 71.45/89.53 & 95.61/85.47 \\
\bottomrule
\end{tabular}
\end{small}
\vspace{-0.3cm}
\end{center}
\caption{\label{result-ngram-zh-table} 
\textcolor{blue}{The performance of fine-tuning Chinese ZEN 2.0 with and without n-gram encoding on different tasks.}
% The performance of Chinese ZEN 2.0 with and without n-gram encoding on 9 Chinese NLP tasks. Only CMRC2018 dataset reports the result of development dataset, the other datasets report the results of test dataset.
}
\vskip -1em
\end{table*}


\begin{table*}[h]
\begin{center}
\begin{small}
\begin{tabular}{p{1.8cm}
                   C{1.3cm} 
                   C{1.55cm} 
                   C{1.6cm}
                   C{1.7cm}
                   C{1.5cm} 
                   C{1.5cm} 
                   C{1.5cm} }
\toprule
\multirow{2}*{\textbf{}}
&\multirow{2}*{\textbf{N-gram}}
&\multicolumn{1}{c}{\textsc{\textbf {ATB}}}
&\multicolumn{1}{c}{\textsc{\textbf{AQMAR}}}
&\multicolumn{1}{c}{\textsc{\textbf{ANERCorp}}}
&\multicolumn{1}{c}{\textsc{\textbf{AR-5}}}
&\multicolumn{1}{c}{\textsc{\textbf{AB-7}}}
&\multicolumn{1}{c}{\textsc{\textbf{KH-7}}}
\\
\addlinespace[0.05cm]
\cline{3-8}
\addlinespace[0.05cm]
~& ~&
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{F1}} & 
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} & 
\multicolumn{1}{c}{\small{ACC}} \\
\midrule	
\multirow{2}*{ZEN 2.0 (B)} & \multicolumn{1}{c}{$\surd$} & \textbf{96.44} & \textbf{79.29} & \textbf{85.83} & \textbf{98.65} & \textbf{96.47} & \textbf{99.03} \\
 & \multicolumn{1}{c}{$\texttimes$} & 96.33 & 78.62 & 84.98 & 98.65 & 96.41 & 98.92 \\
\midrule
\multirow{2}*{ZEN 2.0 (L)} & \multicolumn{1}{c}{$\surd$} & \textbf{96.54} & \textbf{81.07} & \textbf{86.04} & \textbf{98.86} & \textbf{96.67} & \textbf{99.25} \\
 & \multicolumn{1}{c}{$\texttimes$} & 96.48 & 80.24 & 85.67 & 98.76 & 96.58 & 99.14 \\
\bottomrule
\end{tabular}
\begin{tabular}{p{1.8cm}
                   C{1.38cm} 
                   C{2.25cm} 
                   C{2.25cm} 
                   C{2.85cm}
                   C{2.85cm} }
\toprule
\multirow{2}*{\textbf{}}
&\multirow{2}*{\textbf{N-gram}}
&\multicolumn{1}{c}{\textsc{\textbf{ASTD}}}
&\multicolumn{1}{c}{\textsc{\textbf{XNLI}}}
&\multicolumn{1}{c}{\textsc{\textbf{Arabic-SQuAD}}}
&\multicolumn{1}{c}{\textsc{\textbf{ARCD}}}
\\
\addlinespace[0.05cm]
\cline{3-6}
\addlinespace[0.05cm]
~& ~& 
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{ACC}} \\
\midrule	
\multirow{2}*{ZEN 2.0 (B)} & \multicolumn{1}{c}{$\surd$} & \textbf{73.33} & \textbf{79.24} & \textbf{43.32/58.39} & \textbf{32.34/64.89} \\
 & \multicolumn{1}{c}{$\texttimes$} & 73.20 & 78.18 & 41.64/57.18 & 30.91/62.62 \\
\midrule
\multirow{2}*{ZEN 2.0 (L)} & \multicolumn{1}{c}{$\surd$} & \textbf{74.27} & \textbf{81.84} & \textbf{46.15/62.36} & \textbf{37.74/69.90} \\
 & \multicolumn{1}{c}{$\texttimes$} & 74.12 & 81.76 & 45.62/61.95 & 34.62/66.13 \\
\bottomrule
\end{tabular}
\end{small}
\vspace{-0.3cm}
\end{center}
\caption{\label{result-ngram-ar-table} 
\textcolor{blue}{The performance of fine-tuning Arabic ZEN 2.0 with and without n-gram encoding on different tasks.}
% All the datasets report the results of test dataset.
}
\vskip -1em
\end{table*}

==> tables/ft_bak.tex <==



\begin{table*}[h]
\begin{center}
\begin{small}
\begin{tabular}{p{3.2cm}
                   C{0.7cm} 
                   C{0.7cm} C{0.7cm}  
                   C{0.7cm} C{0.7cm} 
                   C{0.9cm} C{0.9cm}
                   C{1.0cm} C{1.0cm} }
\toprule
\multirow{3}*{\textbf{Models}}
&\multicolumn{1}{c}{\textsc{\textbf {MSR-CWS}}}
&\multicolumn{2}{c}{\textsc{\textbf{CTB5}}}
&\multicolumn{2}{c}{\textsc{\textbf{MSRA-NER}}}
&\multicolumn{2}{c}{\textsc{\textbf{THUCNews}}}
&\multicolumn{2}{c}{\textsc{\textbf{ChnSentiCorp}}}\\
\addlinespace[0.05cm]
\cline{2-10}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} \\
\addlinespace[0.05cm]
\cline{2-10}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{F1}} & \multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{F1}} & \multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{ACC}} & \multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} & \multicolumn{1}{c}{\small{ACC}} \\
\midrule	
ERNIE 1.0 (B) & - & - & - & 95.00 & 93.80 & - & - & 95.20 & 95.40 \\
ERNIE 2.0 (B) & & & & & & & & & \\
NEZHA (B) & & & & & & & & &  \\
NEZHA-WWM (B) & & & & & & & & &  \\
K-BERT & & & & & & & & &  \\
\midrule
ERNIE 2.0 (L) & & & & & & & & &  \\
NEZHA (L) & & & & & & & & &  \\
NEZHA-wwm (L) & & & & & & & & &  \\
\midrule
ZEN 1.0 (B) & & & & & & & & &  \\
ZEN 2.0 (B) & & & & & & & & &  \\
ZEN 2.0 (L) & & & & & & & &  \\
\bottomrule
\end{tabular}
\begin{tabular}{p{3.0cm}
                   C{0.6cm} C{0.6cm} 
                   C{0.6cm} C{0.6cm} 
                   C{0.6cm} C{0.6cm} 
                   C{1.0cm} 
                   C{1.3cm} C{1.3cm} }
\toprule
\multirow{3}*{\textbf{Models}}
&\multicolumn{2}{c}{\textsc{\textbf{LCQMC}}}
&\multicolumn{2}{c}{\textsc{\textbf{BQ Corpus}}}
&\multicolumn{2}{c}{\textsc{\textbf{NLI}}}
&\multicolumn{1}{c}{\textsc{\textbf{CMRC2018}}}
&\multicolumn{2}{c}{\textsc{\textbf{NLPCC-DBQA}}}\\
\addlinespace[0.05cm]
\cline{2-10}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} \\
\addlinespace[0.05cm]
\cline{2-10}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{ACC}} & \multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} & \multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} & \multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{EM/F1}} &
\multicolumn{1}{c}{\small{MRR/F1}} & \multicolumn{1}{c}{\small{MRR/F1}} \\
\midrule	
ERNIE 1.0 (B) & 89.70 & 87.40 & 86.10 & 84.80 & 79.90 & 78.40 & 65.10/85.10 & 95.00/82.30 & 95.10/82.70 \\
ERNIE 2.0 (B) & 90.90 & 87.90 & 86.40 & 85.00 & & & & & \\
NEZHA (B) & & & & & & & & &  \\
NEZHA-WWM (B) & & & & & & & & &  \\
K-BERT (B) & & & & & & & & &  \\
\midrule
ERNIE 2.0 (L) & 90.90 & 87.90 & 86.50 & 85.20 & & & & &  \\
NEZHA (L) & & & & & & & & &  \\
NEZHA-wwm (L) & & & & & & & & &  \\
\midrule
ZEN 1.0 (B) & & & & & & & & &  \\
ZEN 2.0 (B) & & & & & & & & &  \\
ZEN 2.0 (L) & & & & & & & &  \\
\bottomrule
\end{tabular}
\end{small}
\vspace{-0.3cm}
\end{center}
\caption{\label{result-zh-table} The overall performance of ZEN and the comparison against previous models on 9 Chinese NLP tasks.}
\vskip -1em
\end{table*}


\begin{table*}[h]
\begin{center}
\begin{small}
\begin{tabular}{p{3.2cm}
                   C{1.2cm} 
                   C{1.2cm} C{1.2cm}
                   C{1.2cm}
                   C{1.2cm} 
                   C{1.2cm} 
                   C{1.2cm} }
\toprule
\multirow{3}*{\textbf{Models}}
&\multicolumn{1}{c}{\textsc{\textbf {PATB}}}
&\multicolumn{2}{c}{\textsc{\textbf{AQMAR}}}
&\multicolumn{1}{c}{\textsc{\textbf{ANERCorp}}}
&\multicolumn{1}{c}{\textsc{\textbf{AR-5}}}
&\multicolumn{1}{c}{\textsc{\textbf{AB-7}}}
&\multicolumn{1}{c}{\textsc{\textbf{KH-7}}}
\\
\addlinespace[0.05cm]
\cline{2-8}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{TEST}} \\
\addlinespace[0.05cm]
\cline{2-8}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{F1}} & \multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{F1}} & 
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} & 
\multicolumn{1}{c}{\small{ACC}} \\
\midrule	
Multi BERT (B) & & & & & & & \\
AraBERT (B) & & & & & & & \\
Arabic BERT (B) & & & & & & & \\
\midrule
ZEN 2.0 (B) & & & & & & & \\
ZEN 2.0 (L) & & & & & & & \\
\bottomrule
\end{tabular}
\begin{tabular}{p{3.2cm}
                   C{1.5cm} 
                   C{1.5cm} 
                   C{1.6cm} C{1.6cm}
                   C{1.6cm} 
                   C{1.6cm} }
\toprule
\multirow{3}*{\textbf{Models}}
&\multicolumn{1}{c}{\textsc{\textbf {ArSAS}}}
&\multicolumn{1}{c}{\textsc{\textbf{ASTD}}}
&\multicolumn{2}{c}{\textsc{\textbf{Arabic-SQuAD}}}
&\multicolumn{1}{c}{\textsc{\textbf{ARCD}}}
&\multicolumn{1}{c}{\textsc{\textbf{XNLI}}}
\\
\addlinespace[0.05cm]
\cline{2-7}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{DEV}} & \multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{TEST}} &
\multicolumn{1}{c}{\small{TEST}} \\
\addlinespace[0.05cm]
\cline{2-7}
\addlinespace[0.05cm]
~& \multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{F1}} & 
\multicolumn{1}{c}{\small{F1}} & \multicolumn{1}{c}{\small{F1}} &
\multicolumn{1}{c}{\small{ACC}} &
\multicolumn{1}{c}{\small{ACC}} \\
\midrule	
Multi BERT (B) & & & & & &  \\
AraBERT (B) & & & & & &  \\
Arabic BERT (B) & & & & & &  \\
\midrule
ZEN 2.0 (B) & & & & & &  \\
ZEN 2.0 (L) & & & & & &  \\
\bottomrule
\end{tabular}
\end{small}
\vspace{-0.3cm}
\end{center}
\caption{\label{result-ar-table} The overall performance of ZEN and the comparison against previous models on 6 Arabic NLP tasks.}
\vskip -1em
\end{table*}
